Understanding Factors that Shape Children's Long Term Engagement with an In-Home Learning Companion Robot

Social robots are emerging as learning companions for children, and research shows that they facilitate the development of interest and learning even through brief interactions. However, little is known about how such technologies might support these goals in authentic environments over long-term periods of use and interaction. We designed a learning companion robot capable of supporting children reading popular-science books by expressing social and informational commentaries. We deployed the robot in homes of 14 families with children aged 10-12 for four weeks during the summer. Our analysis revealed critical factors that affected children's long-term engagement and adoption of the robot, including external factors such as vacations, family visits, and extracurricular activities; family/parental involvement; and children's individual interests. We present four in-depth cases that illustrate these factors and demonstrate their impact on children's reading experiences and discuss the implications of our findings for robot design.

==> IDC2022 - STEMMates/fig_individualreading.tex <==
\begin{figure*}[t!]
    \includegraphics[width=2.9in]{Figures/total_reading_time.pdf}
  \includegraphics[width=2.9in]{Figures/user_book_ratio.pdf}
%   \vspace{-12pt}
  \caption{ Two graphs displaying children's \textit{individual} performance with the books throughout the study, identified by the aliases of each child. The graph on the (left) presents the total minutes each child read to the robot in four weeks. The graph on the (right) presents the number of books read by each child, and the ratio of the book's completion/incompletion rates.
  }
  \label{fig:individual}
%   \vspace{-6pt}
\end{figure*}




==> IDC2022 - STEMMates/fig_interactionflow.tex <==
\begin{figure*}[b!]
  \includegraphics[width=\linewidth]{Figures/interaction_flow.pdf}
%   \vspace{-12pt}
  \caption{\textit{Descriptive illustration of the interaction flow with the robot:} The interaction flow consists of five phases, 1) wake up, 2) identification, 3) book recommendation, 4) reading, 5) interaction termination. A successful interaction with the robot is considered when a child goes through each of these phases, regardless of how long they read with the robot. 
  }
  \label{fig:flow}
%   \vspace{-6pt}
\end{figure*}


==> IDC2022 - STEMMates/fig_overallreading.tex <==
\begin{figure*}[t!]
  \includegraphics[width=2.8in]{Figures/average_book_pages_read.pdf}
    \includegraphics[width=2.8in]{Figures/total_book_counts.pdf}
%   \vspace{-6pt}
  \caption{ Two graphs displaying children's \textit{overall} performance with the books throughout the study. The names of the books and their corresponding page numbers are presented in parenthesis. The graph on the (left) presents the percentage of pages read per book by all children. The graph on the (right) presents the number of times each book has been read by all children, and the ratio of the book's completion/incompletion rates.
  }
  \label{fig:booksread}
  \vspace{-6pt}
\end{figure*}


==> IDC2022 - STEMMates/fig_results.tex <==
\begin{figure*}[t!]
  \includegraphics[width=\linewidth]{Figures/results.pdf}
%   \vspace{-12pt}
  \caption{\textit{Summary of results:} We identified critical factors that impacted children's long term engagement with the robot. Based on children's observed behaviors derived from these critical factors, we categorized children in four cases: Children who 1) modified their interaction 2) discontinued the use of technology 3) were interrupted 4) adopted the technology. %We present descriptive profiles for each child and describe their experiences that led them to each case.
  }
  \label{fig:results}
%   \vspace{-6pt}
\end{figure*}


==> IDC2022 - STEMMates/teaser.tex <==
\begin{figure*}[h!]
    \centering
%   \vspace{-12pt}
% \includegraphics[width=\columnwidth]{Figures/robot_closeup.JPG}
  \includegraphics[height=1.8in]{Figures/robot_closeup.JPG}
    \includegraphics[height=1.8in]{Figures/child_reading.jpg}
%   \vspace{-8pt}
  \caption{Our work explores the factors that shaped children's long-term engagement with a learning companion robot. Children read aloud informal science books to the robot for four weeks during the summer, in their own homes. The robot supported the reading experience by expressing knowledge, social, and interest comments as the child read to the robot. We report the factors that shaped children's reading habits and experiences with the robot and how it changed over time.}
  \label{fig:teaser}
  \vspace{-6pt}
\end{figure*}


==> fig_individualreading.tex <==
\begin{figure*}[t!]
    \includegraphics[width=2.9in]{Figures/total_reading_time.pdf}
  \includegraphics[width=2.9in]{Figures/user_book_ratio.pdf}
%   \vspace{-12pt}
  \caption{ Two graphs displaying children's \textit{individual} performance with the books throughout the study, identified by the aliases of each child. The graph on the (left) presents the total minutes each child read to the robot in four weeks. The graph on the (right) presents the number of books read by each child, and the ratio of the book's completion/incompletion rates.
  }
  \label{fig:individual}
%   \vspace{-6pt}
\end{figure*}



